Lessons from Computational Modelling of Reference Production in Mandarin and English

Referring expression generation (REG) algorithms offer computational models of the production of referring expressions. In earlier work, a corpus of referring expressions (REs) in Mandarin was introduced. In the present paper, we annotate this corpus, evaluate classic REG algorithms on it, and compare the results with earlier results on the evaluation of REG for English referring expressions. Next, we offer an in-depth analysis of the corpus, focusing on issues that arise from the grammar of Mandarin. We discuss shortcomings of previous REG evaluations that came to light during our investigation and we highlight some surprising results. Perhaps most strikingly, we found a much higher proportion of under-specified expressions than previous studies had suggested, not just in Mandarin but in English as well.

==> backup.tex <==
\section{Background}

The analysis reported in paper is based on the \textsc{mtuna} (for Mandarin) and \textsc{etuna} (for English) corpus. We start by briefly introducing the \textsc{tuna} experiments in general, and we highlight some special features of \textsc{mtuna} together with its initial findings.

\subsection{The \textsc{tuna} Experiments}

\textsc{tuna}~\citep{gatt2007evaluating, van2007evaluating} is a series of controlled elicitation experiments that were set up to facilitate computational linguist's understanding of human reference production. In particular, the corpora to which these experiments gave rise, were employed to evaluate REG algorithms, by comparing their output with the REs in these corpora. The stimuli in the \textsc{tuna} experiments were divided into two types of visual scenes: scenes that depict furniture and scenes that depict people. Figure~\ref{fig:tuna} shows an example for each of these two types of scenes. In each trial, one or two objects in the scene were chosen as the target referent(s), demarcated by red borders. The subjects were asked to produce referring expressions that identify the target referents from the other objects in the scene (their ``distractors"). The trials in the people domain were more challenging than those in the furniture domain because 1) the people domain uses real (black and white) photographs while furniture domain use synthetic pictures; and 2) the images in the people domain are arguably more perceptually similar to each other. % KvD Do we need to say this?

% KvD The following was revised:
The resulting corpus, which we will call \textsc{etuna}, was subsequently studied for evaluating a set of ``classic'' REG algorithms~\citep{deemter2012generation}. Although RE has given rise to a good number of other corpora, with subtly different qualities (e.g., .... ADD ...), we focus here on the TUNA corpora for two reasons: firstly the \textsc{etuna} corpus was used in a series of Shared Task Evaluation Campaign~\citep{gatt2010introducing}, which caused it to be relatively well known. Secondly and more importantly from the perspective of the present paper, \textsc{etuna} was used as a blueprint for a number of similarly constructed corpora for the study of reference in other languages, namely Dutch~\citep[\textsc{dtuna},][]{koolen2010d}, Germany~\citep[\textsc{gtuna},][]{howcroft2017g}, and Mandarin~\citep{van-deemter-etal-2017-investigating}.

\subsection{The Mandarin \textsc{tuna}} \label{sec:mtuna}

% KvD I've tentatively added the following. Can we do better?
The different TUNA corpora were set up in highly similar fashion: for instance, they all use a few dozen stimuli, each of which was offered in isolation (i.e., previous scenes, and previous utterances, had to be disregarded), and which were chosen from the same sets of furniture and people images, and participants were asked to enter a type-written RE following a question. Yet there were subtle differences between these corpora as well, reflecting specific research questions that the various sets of authors had with the corpus.

The stimuli used by \textsc{mtuna} were inherited from the \textsc{dtuna}, where there are totally 40 trials. Different from other \textsc{tuna}s where they always asked subjects essentially the same question, namely \emph{Which object/objects appears/appear in a red window?}, the new experiment distinguished between referring expressions in subject and object position.\footnote{This was done because 
the literature on Mandarin (e.g., REF Chao 1968) suggests that Mandarin NPs in pre-verbal position may be interpreted as definite unless there is information to the contrary.}
More precisely, subjects were asked to fill referring expressions in blanks in either of the following patterns: 
\ex. \a. \_\_\_\_ 在红色方块中
    \glt `Please complete the sentence: \_\_\_\_ is in the red frame(s)'
     \b. 红色方块中的是 \_\_\_\_ 
    \glt `What’s in the red frame is \_\_\_\_'

where (a) asked subjects to place the referring expression in subject position while (b) asked to place it in object position. 

% Guanyi: Is this the thing you want to see in this section? 
% KvD Yes, but I think we also need to (1) say something about the idea behind all the TUNAs (see tentative addition above), and (2) explain why MTUNA distinguishes between subject and object. (See the footnote that I've added.)

The initial analysis addressed in \citet{van-deemter-etal-2017-investigating} focused on how definiteness was expressed in Mandarin REs, i.e., are those REs definite or indefinite and definite REs are expressed in which canonical form? They concluded that 1) most definite REs are bare nouns\footnote{Mandarin is thought not to use any definiteness markers (like the articles in English, for instance).}; 2) indefinite REs also appears quite often, most of which appears in the subject position. They also have a look at how often the markers for number (i.e., the number of the objects that the speaker refers to), maximality (i.e., is the speaker talking about one of the targets or both of them?) and givenness (i.e., is the speaker talking about something that the hearer familiar with?) appears to have a preliminary understanding on whether Mandarin prefers brevity than clarity as they hypothesised. % KvD The previous sentence is difficult to follow.
As expected, they found some very in-frequently used maximality marker (i.e., 都 (all)) and no number and giveness markers were found. % KvD Do we need to say this? If we do, we need to explain why this is important.
